Circular-arc graphs and the Helly property

In this paper we investigate some problems related to the Helly properties of circular-arc graphs, which are defined as intersection graphs of arcs of a fixed circle. As such, circular-arc graphs are among the simplest classes of intersection graphs whose models might not satisfy the Helly property. In particular, some cliques of a circular-arc graph might be Helly in some but not all arc intersection models of the graph. Our first result is an alternative proof of a theorem by Lin and Szwarcfiter which asserts that for every circular-arc graph $G$ either every normalized model of $G$ satisfies the Helly property or no normalized model of $G$ satisfies this property. Further, we study the Helly properties of a single clique of a circular-arc graph $G$. We divide the cliques of $G$ into three types: a clique $C$ of $G$ is always-Helly/always-non-Helly/ambiguous if $C$ is Helly in every/no/(some but not all) normalized model of $G$. We provide a combinatorial description for the cliques of each type, and based on it, we devise a polynomial time algorithm which determines the type of a given clique. Finally, we study the Helly Cliques problem, in which we are given an $n$-vertex circular-arc graph $G$ and some of its cliques $C_1, \ldots, C_k$ and we ask if there is an arc intersection model of $G$ in which all the cliques $C_1, \ldots, C_k$ satisfy the Helly property. We show that: (1) the Helly Cliques problem admits a $2^{O(k\log{k})}n^{O(1)}$-time algorithm (that is, it is FPT when parametrized by the number of cliques given in the input), (2) assuming Exponential Time Hypothesis (ETH), the Helly Cliques problem cannot be solved in time $2^{o(k)}n^{O(1)}$, (3) the Helly Cliques problem admits a polynomial kernel of size $O(k^6)$. All our results use a data structure, called a PQM-tree, which maintains all normalized models of a circular-arc graph $G$.

==> figures/data_structure/admissible_models_correspondence.tex <==
\begin{figure}[ht]
\begin{tikzpicture}[scale=0.8,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\tikzstyle{every node}=[rectangle,minimum size=15pt,inner sep=0.5,draw];
  \begin{scriptsize}
  \node (M) at (4.0,7.5) {$S_i$};
  \node (v1) at (0.5,6) {$A_1 = \{v_1\}$};
  \node (A) at (3,6) {$A_2$};
  \node (B) at (5.5,6) {$A_3$};
  \node (v9) at (8,6) {$A_4 = \{v_9\}$};
  \node (v2) at (0.5,4.5) {$B_1 = \{v_2\}$};
  \node (C) at (2.5,4.5) {$B_2$};
  \node (D) at (4,4.5) {$B_3$};
  \node (v7) at (5.5,4.5) {$\{v_7\}$};
  \node (v8) at (7,4.5) {$\{v_8\}$};
  \node (v3) at (1.8,3) {$\{v_3\}$};
  \node (v4) at (2.8,3) {$\{v_4\}$};
  \node (v5) at (4.0,3) {$\{v_5\}$};
  \node (v6) at (5,3) {$\{v_6\}$};
 
\end{scriptsize}
\tikzstyle{every node}=[rectangle,minimum size=15pt,inner sep=0.5,draw];
\path (M) edge (v1); 
\path (M) edge (A); 
\path (M) edge (B); 
\path (M) edge (v9); 
\path (A) edge (v2); 
\path (A) edge (C); 
\path (A) edge (D); 
\path (B) edge (v7); 
\path (B) edge (v8); 
\path (C) edge (v3); 
\path (C) edge (v4); 
\path (D) edge (v5); 
\path (D) edge (v6); 

\draw[-,white] (-0.5,1) -- (0,1);
\end{tikzpicture}
\hspace{0.5cm}
\begin{tikzpicture}[xscale=0.75,yscale=0.75,>=latex,shorten>=-0.2pt,shorten <=-0.2pt]
\coordinate (a_v1) at (0,3) {};
\coordinate (a_v2) at (1,3) {};
\coordinate (a_v3) at (2,3) {};
\coordinate (a_v4) at (2.5,3) {};
\coordinate (a_v5) at (3.4,3) {};
\coordinate (a_v6) at (3.8,3) {};
\coordinate (a_v7) at (5.2,3) {};
\coordinate (a_v8) at (5.8,3) {};
\coordinate (a_v9) at (7,3) {};

\coordinate (b_v2) at (7,0) {};
\coordinate (b_v4) at (6,0) {};
\coordinate (b_v3) at (5.5,0) {};
\coordinate (b_v6) at (4.5,0) {};
\coordinate (b_v5) at (4.1,0) {};
\coordinate (b_v9) at (2.5,0) {};
\coordinate (b_v1) at (1.5,0) {};
\coordinate (b_v8) at (0.6,0) {};
\coordinate (b_v7) at (0,0) {};

\coordinate (lb_v2) at (7,-0.3) {};
\coordinate (lb_v4) at (6,-0.3) {};
\coordinate (lb_v3) at (5.5,-0.3) {};
\coordinate (lb_v6) at (4.5,-0.3) {};
\coordinate (lb_v5) at (4.1,-0.3) {};
\coordinate (lb_v9) at (2.5,-0.3) {};
\coordinate (lb_v1) at (1.5,-0.3) {};
\coordinate (lb_v8) at (0.6,-0.3) {};
\coordinate (lb_v7) at (0,-0.3) {};


\coordinate (tau0) at (7.9,3);
\coordinate (tau1) at (-0.9,0);


\tikzstyle{every node}=[inner sep=2pt,fill=white]

\draw[fill=gray!30, draw=none] (-0.2,3) -- (0.2,3) -- (1.7,0) -- (1.3,0) -- cycle;
\coordinate (m_A1) at (0,3.3) {};

\draw[fill=gray!30, draw=none] (0.7,3) -- (4.1,3) -- (7.3,0) -- (3.8,0) -- cycle;
\coordinate (m_A) at (5.55,-0.3) {};

\draw[fill=gray!30, draw=none] (4.9,3) -- (6.1,3) -- (0.9,0) -- (-0.3,0) -- cycle;
\coordinate (m_A3) at (5.5,3.3) {};

\draw[fill=gray!30, draw=none] (6.7,3) -- (7.3,3) -- (2.8,0) -- (2.2,0) -- cycle;
\coordinate (m_A4) at (7,3.3) {};

\draw[fill=gray!80, draw=none] (0.7,3) -- (1.3,3) -- (7.3,0) -- (6.7,0) -- cycle;
\coordinate (m_B1) at (1,3.3) {};
\draw[fill=gray!80, draw=none] (1.8,3) -- (2.7,3) -- (6.2,0) -- (5.3,0) -- cycle;
\coordinate (m_B2) at (2.25,3.3) {};
\draw[fill=gray!80, draw=none] (3.2,3) -- (4,3) -- (4.7,0) -- (3.9,0) -- cycle;
\coordinate (m_B3) at (3.7,3.3) {};

\draw[<-] (a_v1)--(b_v1);
\draw[->] (a_v2)--(b_v2);
\draw[<-] (a_v3)--(b_v3);
\draw[->] (a_v4)--(b_v4);
\draw[<-] (a_v5)--(b_v5);
\draw[->] (a_v6)--(b_v6);
\draw[<-] (a_v7)--(b_v7);
\draw[->] (a_v8)--(b_v8);
\draw[->] (a_v9)--(b_v9);

\draw[->] (-0.5,3) -- (7.5,3);
\draw[<-] (-0.5,0) -- (7.5,0);


\tikzstyle{every node}=[inner sep=1pt]
\begin{footnotesize}
\node at (lb_v1) {$v_1$};
\node at (lb_v2) {$v_2$};
\node at (lb_v3) {$v_3$};
\node at (lb_v4) {$v_4$};
\node at (lb_v5) {$v_5$};
\node at (lb_v6) {$v_6$};
\node at (lb_v7) {$v_7$};
\node at (lb_v8) {$v_8$};
\node at (lb_v9) {$v_9$};
\node at (tau0) {$\mu^0$};
\node at (tau1) {$\mu^1$};
\node at (m_A1) {$A_1$};
\node at (m_B1) {$B_1$};
\node at (m_B2) {$B_2$};
\node at (m_B3) {$B_3$};
\node at (m_A3) {$A_3$};
\node at (m_A4) {$A_4$};
%\node at (m_v9) {$\{v_9\}$};

\end{footnotesize}

%gorna kopia
\coordinate (a_v1) at (0,5) {};
\coordinate (a_v2) at (1,5) {};
\coordinate (a_v3) at (2,5) {};
\coordinate (a_v4) at (2.5,5) {};
\coordinate (a_v5) at (3.4,5) {};
\coordinate (a_v6) at (3.8,5) {};
\coordinate (a_v7) at (5.2,5) {};
\coordinate (a_v8) at (5.8,5) {};
\coordinate (a_v9) at (7,5) {};


\coordinate (b_v2) at (7,8) {};
\coordinate (b_v4) at (6,8) {};
\coordinate (b_v3) at (5.5,8) {};
\coordinate (b_v6) at (4.5,8) {};
\coordinate (b_v5) at (4.1,8) {};
\coordinate (b_v9) at (2.5,8) {};
\coordinate (b_v1) at (1.5,8) {};
\coordinate (b_v8) at (0.6,8) {};
\coordinate (b_v7) at (0,8) {};

\coordinate (la_v1) at (0,4.7) {};
\coordinate (la_v2) at (1,4.7) {};
\coordinate (la_v3) at (2,4.7) {};
\coordinate (la_v4) at (2.5,4.7) {};
\coordinate (la_v5) at (3.4,4.7) {};
\coordinate (la_v6) at (3.8,4.7) {};
\coordinate (la_v7) at (5.2,4.7) {};
\coordinate (la_v8) at (5.8,4.7) {};
\coordinate (la_v9) at (7,4.7) {};

\coordinate (mu0) at (-0.9,5);
\coordinate (mu1) at (7.9,8);

\tikzstyle{every node}=[inner sep=2pt,fill=white]

\draw[fill=gray!30, draw=none] (-0.2,5) -- (0.2,5) -- (1.7,8) -- (1.3,8) -- cycle;
\coordinate (m_A1) at (1.5,8.3) {};

\draw[fill=gray!30, draw=none] (0.7,5) -- (4.1,5) -- (7.3,8) -- (3.8,8) -- cycle;
%\coordinate (m_A) at (2.4,4.7) {};

\draw[fill=gray!30, draw=none] (4.9,5) -- (6.1,5) -- (0.9,8) -- (-0.3,8) -- cycle;
\coordinate (m_A2) at (0.3,8.3) {};

\draw[fill=gray!30, draw=none] (6.7,5) -- (7.3,5) -- (2.8,8) -- (2.2,8) -- cycle;
\coordinate (m_A3) at (2.5,8.3) {};

\draw[fill=gray!80, draw=none] (0.7,5) -- (1.3,5) -- (7.3,8) -- (6.7,8) -- cycle;
\coordinate (m_B1) at (7,8.3) {};
\draw[fill=gray!80, draw=none] (1.8,5) -- (2.7,5) -- (6.2,8) -- (5.3,8) -- cycle;
\coordinate (m_B2) at (5.75,8.3) {};
\draw[fill=gray!80, draw=none] (3.2,5) -- (4,5) -- (4.7,8) -- (3.9,8) -- cycle;
\coordinate (m_B3) at (4.3,8.3) {};


\draw[->] (a_v1)--(b_v1);
\draw[<-] (a_v2)--(b_v2);
\draw[->] (a_v3)--(b_v3);
\draw[<-] (a_v4)--(b_v4);
\draw[->] (a_v5)--(b_v5);
\draw[<-] (a_v6)--(b_v6);
\draw[->] (a_v7)--(b_v7);
\draw[<-] (a_v8)--(b_v8);
\draw[<-] (a_v9)--(b_v9);

\draw[<-] (-0.5,5) -- (7.5,5);
\draw[->] (-0.5,8) -- (7.5,8);

\tikzstyle{every node}=[inner sep=1pt]
\begin{footnotesize}
\node at (la_v1) {$v_1$};
\node at (la_v2) {$v_2$};
\node at (la_v3) {$v_3$};
\node at (la_v4) {$v_4$};
\node at (la_v5) {$v_5$};
\node at (la_v6) {$v_6$};
\node at (la_v7) {$v_7$};
\node at (la_v8) {$v_8$};
\node at (la_v9) {$v_9$};
\node at (mu0) {$\tau^1$};
\node at (mu1) {$\tau^0$};
\node at (m_A1) {$A_1$};
\node at (m_A2) {$A_3$};
\node at (m_A3) {$A_4$};
\node at (m_B1) {$B_1$};
\node at (m_B2) {$B_2$};
\node at (m_B3) {$B_3$};
\end{footnotesize}

\end{tikzpicture}
\caption{\label{fig:admissible_models_modular_decomposition} Modular decomposition $\strongModules(S_i,{\sim})$ of $(S_i,{\sim})$ (to the left) 
and two admissible models for $\mathbb{S}_i$ (to the right).
Module $S_i$ is prime and hence the set $\Pi(S_i)$ contains two transitive orientations of $(S_i,{\sim_{S_i}})$.
Module $A_2$ is serial with three children and hence the set $\Pi(A_2)$ has $3!$ transitive orientations of $(A_2,{\sim_{A_2}})$.
The remaining non-trivial modules $A_3, B_2, B_3$ are parallel and hence each of the sets $\Pi(A_3)$, $\Pi(B_2)$, and $\Pi(B_3)$ contains one empty transitive orientation of 
$(A_3,{\sim_{A_3}})$, $(B_2,{\sim_{B_2}})$, and $(B_3,{\sim_{B_3}})$, respectively.
Hence, the metachord $\mathbb{S}_i$ has $12$ different admissible models, corresponding to $12=2 \cdot 3!$ transitive orientations of $(S_i,{\sim})$.
}
\end{figure}


==> figures/forb_structures.tex <==
\begin{tikzpicture}[scale=0.45,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\label{fig:forb_structures}
\coordinate (center) at (0,0) {};
\coordinate (label) at (0,-2.5) {};

\coordinate (s1) at ($(center)+(0:2.0cm)$) {};
\coordinate (s2) at ($(center)+(60:2.0cm)$) {};
\coordinate (s3) at ($(center)+(120:2.0cm)$) {};
\coordinate (s4) at ($(center)+(180:2.0cm)$) {};
\coordinate (s5) at ($(center)+(240:2.0cm)$) {};
\coordinate (s6) at ($(center)+(300:2.0cm)$) {};


\node at ($(center)+(0:2.7cm)$) {$v_0^0$};
\node at ($(center)+(60:2.7cm)$) {$v_1^1$};
\node at ($(center)+(120:2.7cm)$) {$v_2^0$};
\node at ($(center)+(180:2.7cm)$) {$v_0^1$};
\node at ($(center)+(240:2.7cm)$) {$v_1^0$};
\node at ($(center)+(300:2.7cm)$) {$v_2^1$};


\draw (0,0) circle (2cm);

\draw[thick,red,->] (s1) -- (s4);
\draw[thick,red,->] (s5) -- (s2);
\draw[thick,red,->] (s3) -- (s6);

%\draw[black] (-2.5,-3)--(-2.5,-3);
%\draw[black] (2.5,3)--(2.5,3);
\draw[white] (-2.5,-2)--(-2.5,-2);
\draw[white] (2.5,2)--(2.5,2);
\end{tikzpicture}
\hspace{0.1cm}
\begin{tikzpicture}[scale=0.5,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (center) at (0,0) {};
\coordinate (label) at (0,-2.5) {};

\coordinate (s1) at ($(center)+(30:2.0cm)$) {};
\coordinate (s2) at ($(center)+(60:2.0cm)$) {};
\coordinate (s3) at ($(center)+(120:2.0cm)$) {};
\coordinate (s4) at ($(center)+(150:2.0cm)$) {};
\coordinate (s5) at ($(center)+(210:2.0cm)$) {};
\coordinate (s6) at ($(center)+(240:2.0cm)$) {};
\coordinate (s7) at ($(center)+(300:2.0cm)$) {};
\coordinate (s8) at ($(center)+(330:2.0cm)$) {};

\node at ($(center)+(30:2.7cm)$) {$v_0^0$};
\node at ($(center)+(60:2.7cm)$) {$v_1^1$};
\node at ($(center)+(120:2.7cm)$) {$v_3^0$};
\node at ($(center)+(150:2.7cm)$) {$v_0^1$};
\node at ($(center)+(210:2.7cm)$) {$v_2^0$};
\node at ($(center)+(240:2.7cm)$) {$v_3^1$};
\node at ($(center)+(300:2.7cm)$) {$v_1^0$};
\node at ($(center)+(330:2.7cm)$) {$v_2^1$};


\draw (0,0) circle (2cm);

\draw[thick,red,->] (s1) -- (s4);
\draw[thick,red,->] (s7) -- (s2);
\draw[thick,red,->] (s3) -- (s6);
\draw[thick,red,->] (s5) -- (s8);

%\draw[black] (-2.5,-3)--(-2.5,-3);
%\draw[black] (2.5,3)--(2.5,3);
\draw[white] (-2.6,-2)--(-2.6,-2);
\draw[white] (2.6,2)--(2.6,2);
\end{tikzpicture}
\hspace{0.1cm}
\begin{tikzpicture}[scale=0.5,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (center) at (0,0) {};
\coordinate (label) at (0,-2.5) {};

\coordinate (s1) at ($(center)+(30:2.0cm)$) {};
\coordinate (s2) at ($(center)+(60:2.0cm)$) {};
\coordinate (s3) at ($(center)+(102:2.0cm)$) {};
\coordinate (s4) at ($(center)+(132:2.0cm)$) {};
\coordinate (s5) at ($(center)+(174:2.0cm)$) {};
\coordinate (s6) at ($(center)+(204:2.0cm)$) {};
\coordinate (s7) at ($(center)+(246:2.0cm)$) {};
\coordinate (s8) at ($(center)+(276:2.0cm)$) {};
\coordinate (s9) at ($(center)+(318:2.0cm)$) {};
\coordinate (s10) at ($(center)+(348:2.0cm)$) {};

\node at ($(center)+(30:2.7cm)$) {$v_0^0$};
\node at ($(center)+(60:2.7cm)$) {$v_1^1$};
\node at ($(center)+(102:2.7cm)$) {$v_4^0$};
\node at ($(center)+(132:2.7cm)$) {$v_0^1$};
\node at ($(center)+(174:2.7cm)$) {$v_3^0$};
\node at ($(center)+(204:2.7cm)$) {$v_4^1$};
\node at ($(center)+(246:2.7cm)$) {$v_2^0$};
\node at ($(center)+(276:2.7cm)$) {$v_3^1$};
\node at ($(center)+(318:2.7cm)$) {$v_1^0$};
\node at ($(center)+(348:2.7cm)$) {$v_2^1$};



\draw (0,0) circle (2cm);

\draw[thick,red,->] (s1) -- (s4);
\draw[thick,red,->] (s7) -- (s10);
\draw[thick,red,->] (s3) -- (s6);
\draw[thick,red,->] (s5) -- (s8);
\draw[thick,red,->] (s9) -- (s2);

\end{tikzpicture}


==> figures/parallel_case/t_nm_tree.tex <==
\begin{figure}[htp!]
\begin{tikzpicture}[scale=1,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (center) at (0,0) {};
\coordinate (label) at (0,-3) {};

\coordinate (m11) at ($(center)+(90:1.95cm)$) {};
\coordinate (m112) at ($(center)+(180:0.5cm)$) {};
\coordinate (m12) at ($(center)+(270:1.98cm)$) {};
\coordinate (m13) at ($(center)+(330:0.5cm)$) {};
\coordinate (m14) at ($(center)+(0:2cm)$) {};
\coordinate (m15) at ($(center)+(30:0.5cm)$) {};
\coordinate (lm1) at ($(center)+(90:2.3cm)$) {};

\coordinate (m21) at ($(center)+(10:2cm)$) {};
\coordinate (m22) at ($(center)+(20:1.8cm)$) {};
\coordinate (m23) at ($(center)+(30:2cm)$) {};
\coordinate (m24) at ($(center)+(20:1.6cm)$) {};
\coordinate (lm2) at ($(center)+(20:2.3cm)$) {};



\coordinate (m31) at ($(center)+(35:2cm)$) {};
\coordinate (m32) at ($(center)+(55:1.5cm)$) {};
\coordinate (m33) at ($(center)+(75:2cm)$) {};
\coordinate (m34) at ($(center)+(55:1cm)$) {};
\coordinate (lm3) at ($(center)+(55:2.3cm)$) {};


\coordinate (m41) at ($(center)+(120:2cm)$) {};
\coordinate (m42) at ($(center)+(0:-1.2cm)$) {};
\coordinate (m43) at ($(center)+(240:2cm)$) {};
\coordinate (m44) at ($(center)+(0:-0.8cm)$) {};
\coordinate (lm4) at ($(center)+(120:2.3cm)$) {};

\coordinate (m51) at ($(center)+(290:2cm)$) {};
\coordinate (m52) at ($(center)+(315:1.7cm)$) {};
\coordinate (m53) at ($(center)+(340:2cm)$) {};
\coordinate (m54) at ($(center)+(315:1.3cm)$) {};
\coordinate (lm5) at ($(center)+(315:2.3cm)$) {};


\coordinate (ln1) at ($(center)+(23:1.1cm)$) {};
\coordinate (ln2) at ($(center)+(112:1.56cm)$) {};
\coordinate (ln3) at ($(center)+(330:1.0cm)$) {};

\coordinate (v) at ($(center)+(270:2.3cm)$) {};


\begin{scriptsize}
\tikzstyle{every node}=[inner sep=1pt]
\node at (lm1) {$Q_1$};
\node at (lm2) {$Q_2$};
\node at (lm3) {$Q_3$};
\node at (lm4) {$Q_4$};
\node at (lm5) {$Q_5$};

\node at (ln1) {$P_1$};
\node at (ln2) {$P_2$};
\node at (ln3) {$P_3$};

\node[red] at (v) {$\phi(v)$};
\end{scriptsize}


%m1
\draw[thick, fill = gray] plot [smooth cycle] coordinates {(m11) (m112) (m12) (m13) (m14) (m15)};

%m2
\draw[thick] plot [smooth cycle] coordinates {(m21) (m22) (m23) (m24)};

%m3
\draw[thick] plot [smooth cycle] coordinates {(m31) (m32) (m33) (m34)};


%m4
\draw[thick] plot [smooth cycle] coordinates {(m41) (m42) (m43) (m44)};

%m5
\draw[thick] plot [smooth cycle] coordinates {(m51) (m52) (m53) (m54)};


\draw[thick] (0,0) circle (2cm);

\draw[<-, red] ($(center)+(90:2cm)$)--($(center)+(270:2cm)$);



\draw[white] (-2.5,-2.5)--(-2.5,-2.3);
\draw[white] (2.5,2.5)--(2.5,2.3);

\end{tikzpicture} 
\hspace{1cm}
\begin{tikzpicture}[scale=0.75,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
  \tikzstyle{every node}=[circle,minimum size=10pt,inner sep=0.5,draw];
  \begin{scriptsize}
  \node (m1) at (0.0,0) {$M_1$};
  \node (m4) at (-2,0.0) {$M_4$};
  \node (m3) at (2,1.5) {$M_3$};
  \node (m2) at (2,0.25) {$M_2$};
  \node (m5) at (2,-1) {$M_5$};
  \end{scriptsize}
  \tikzstyle{every node}=[square,minimum size=15pt,inner sep=0.5,draw];
  \begin{scriptsize}
  \node (n1) at (0.75,1.0) {$N_1$};
  \node (n3) at (0.75,-1.0) {$N_3$};
  \node (n2) at (-1.0,0) {$N_2$};
  \end{scriptsize}
\path (m1) edge (n1); 
\path (m1) edge (n2); 
\path (m1) edge (n3); 

\path (n1) edge (m3); 
\path (n1) edge (m2); 
\path (n3) edge (m5); 
\path (m4) edge (n2); 

\draw[white] (-2.5,-2.4)--(-2.5,-1.8);
\draw[white] (2.5,2.6)--(2.5,2.3);
\end{tikzpicture}
\caption{\label{fig:T_NM_tree} To the left: a schematic view of 
a conformal model $\phi$ of~$G_{ov}$ in which every module $M$ is represented by a closed curve encompassing all the chords from $\phi(M)$ 
and touching the circle $C$ in points where the chords of $\phi(M)$ intersect $C$. 
To the right: $T_{\mathcal{NM}}$ tree with the nodes
$N_1,N_2,N_3$ and the modules $M_1,M_2,M_3,M_4,M_5$.
Vertex $v$ separates $M_4$ from $M_2,M_3,M_5$.
The maximal subsets consisting of pairwise inseparated modules are $\{M_1,M_2,M_3\}$, $\{M_1,M_4\}$, and $\{M_1,M_5\}$,
which correspond to the nodes $N_1$, $N_2$, and $N_3$, respectively.
}
\end{figure}


==> figures/parallel_case/t_nm_tree_subwords.tex <==
\begin{figure}[htp!]
\begin{tikzpicture}[scale=1,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (m11) at ($(center)+(90:1.95cm)$) {};
\coordinate (m112) at ($(center)+(180:0.5cm)$) {};
\coordinate (m12) at ($(center)+(270:1.98cm)$) {};
\coordinate (m13) at ($(center)+(330:0.5cm)$) {};
\coordinate (m14) at ($(center)+(0:2cm)$) {};
\coordinate (m15) at ($(center)+(30:0.5cm)$) {};
\coordinate (lm1) at ($(center)+(90:0.0cm)$) {};
\coordinate (phi_m1) at ($(center)+(225:2.07cm)$) {};

\coordinate (m21) at ($(center)+(10:2cm)$) {};
\coordinate (m22) at ($(center)+(20:1.8cm)$) {};
\coordinate (m23) at ($(center)+(30:2cm)$) {};
\coordinate (m24) at ($(center)+(20:1.6cm)$) {};
\coordinate (lm2) at ($(center)+(10:1.5cm)$) {};
\coordinate (phi_m2) at ($(center)+(20:2.05cm)$) {};



\coordinate (m31) at ($(center)+(35:2cm)$) {};
\coordinate (m32) at ($(center)+(55:1.5cm)$) {};
\coordinate (m33) at ($(center)+(75:2cm)$) {};
\coordinate (m34) at ($(center)+(55:1cm)$) {};
\coordinate (lm3) at ($(center)+(55:1.8cm)$) {};


\coordinate (m41) at ($(center)+(120:2cm)$) {};
\coordinate (m42) at ($(center)+(0:-1.2cm)$) {};
\coordinate (m43) at ($(center)+(240:2cm)$) {};
\coordinate (m44) at ($(center)+(0:-0.8cm)$) {};
\coordinate (lm4) at ($(center)+(180:1.5cm)$) {};

\coordinate (m51) at ($(center)+(290:2cm)$) {};
\coordinate (m52) at ($(center)+(315:1.7cm)$) {};
\coordinate (m53) at ($(center)+(340:2cm)$) {};
\coordinate (m54) at ($(center)+(315:1.3cm)$) {};
\coordinate (lm5) at ($(center)+(285:1.7cm)$) {};


\coordinate (ln1) at ($(center)+(26:1.1cm)$) {};
\coordinate (ln2) at ($(center)+(112:1.56cm)$) {};
\coordinate (ln3) at ($(center)+(330:1.0cm)$) {};


%\draw[very thick,red,|-|] ([shift=(10:2cm)]0,0) arc (10:75:2cm);
\coordinate (phi_n1) at ($(center)+(42.5:2.1cm)$) {};

%\draw[very thick,red,|-|] ([shift=(85:2cm)]0,0) arc (85:95:2cm);
\coordinate (phi_tau_1) at ($(center)+(90:2.25cm)$) {};

%\draw[very thick,red,|-|] ([shift=(120:2cm)]0,0) arc (120:240:2cm);
\coordinate (phi_n2) at ($(center)+(225:2.1cm)$) {};

%\draw[very thick,red,|-|] ([shift=(265:2cm)]0,0) arc (265:275:2cm);
\coordinate (phi_tau_2) at ($(center)+(270:2.25cm)$) {};

%\draw[very thick,red,|-|] ([shift=(290:2cm)]0,0) arc (290:340:2cm);
\coordinate (phi_n3) at ($(center)+(315:2.1cm)$) {};

%\draw[very thick,red,|-|] ([shift=(-5:2cm)]0,0) arc (-5:5:2cm);
\coordinate (phi_tau_3) at ($(center)+(0:2.25cm)$) {};


\begin{tiny}
\tikzstyle{every node}=[inner sep=1pt]
\node[anchor=west] at (phi_n1) {$\phi|V_{T\setminus M_1}(N_1)$};
\node[anchor=east] at (phi_n2) {$\phi|V_{T\setminus M_1}(N_2)$};
\node[anchor=west] at (phi_n3) {$\phi|V_{T\setminus M_1}(N_3)$};
\node at (phi_tau_1) {$\tau_1$};
\node at (phi_tau_2) {$\tau_3$};
\node at (phi_tau_3) {$\tau_2$};



\node at (lm1) {$M_1$};
\node at (lm2) {$M_2$};

\node at (lm3) {$M_3$};

\node at (lm4) {$M_4$};
\node at (lm5) {$M_5$};

\node at (ln1) {$N_1$};
\node at (ln2) {$N_2$};
\node at (ln3) {$N_3$};
\end{tiny}


%m1
\draw[thick] plot [smooth cycle] coordinates {(m11) (m112) (m12) (m13) (m14) (m15)};

%m2
\draw[thick] plot [smooth cycle] coordinates {(m21) (m22) (m23) (m24)};

%m3
\draw[thick] plot [smooth cycle] coordinates {(m31) (m32) (m33) (m34)};


%m4
\draw[thick] plot [smooth cycle] coordinates {(m41) (m42) (m43) (m44)};

%m5
\draw[thick] plot [smooth cycle] coordinates {(m51) (m52) (m53) (m54)};


\draw (0,0) circle (2cm);

\draw[very thick,red,|-|] ([shift=(10:2cm)]0,0) arc (10:75:2cm);

\draw[very thick,red,|-|] ([shift=(85:2cm)]0,0) arc (85:95:2cm);

\draw[very thick,red,|-|] ([shift=(120:2cm)]0,0) arc (120:240:2cm);

\draw[very thick,red,|-|] ([shift=(265:2cm)]0,0) arc (265:275:2cm);

\draw[very thick,red,|-|] ([shift=(290:2cm)]0,0) arc (290:340:2cm);

\draw[very thick,red,|-|] ([shift=(-5:2cm)]0,0) arc (-5:5:2cm);

\draw[white] (-3.4,-2.5)--(-3.4,-2.3);
\draw[white] (3.8,2.5)--(3.8,2.3);

\end{tikzpicture} 
\hspace{0.5cm}
\begin{tikzpicture}[scale=1,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (m11) at ($(center)+(90:1.95cm)$) {};
\coordinate (m112) at ($(center)+(180:0.5cm)$) {};
\coordinate (m12) at ($(center)+(270:1.98cm)$) {};
\coordinate (m13) at ($(center)+(330:0.5cm)$) {};
\coordinate (m14) at ($(center)+(0:2cm)$) {};
\coordinate (m15) at ($(center)+(30:0.5cm)$) {};
\coordinate (lm1) at ($(center)+(90:0.0cm)$) {};
\coordinate (phi_m1) at ($(center)+(225:2.07cm)$) {};

\coordinate (m21) at ($(center)+(10:2cm)$) {};
\coordinate (m22) at ($(center)+(20:1.8cm)$) {};
\coordinate (m23) at ($(center)+(30:2cm)$) {};
\coordinate (m24) at ($(center)+(20:1.6cm)$) {};
\coordinate (lm2) at ($(center)+(10:1.5cm)$) {};
\coordinate (phi_m2) at ($(center)+(20:2.05cm)$) {};



\coordinate (m31) at ($(center)+(35:2cm)$) {};
\coordinate (m32) at ($(center)+(55:1.5cm)$) {};
\coordinate (m33) at ($(center)+(75:2cm)$) {};
\coordinate (m34) at ($(center)+(55:1cm)$) {};
\coordinate (lm3) at ($(center)+(55:1.8cm)$) {};
\coordinate (phi_m3) at ($(center)+(55:2.1cm)$) {};


\coordinate (m41) at ($(center)+(120:2cm)$) {};
\coordinate (m42) at ($(center)+(0:-1.2cm)$) {};
\coordinate (m43) at ($(center)+(240:2cm)$) {};
\coordinate (m44) at ($(center)+(0:-0.8cm)$) {};
\coordinate (lm4) at ($(center)+(180:1.5cm)$) {};

\coordinate (m51) at ($(center)+(290:2cm)$) {};
\coordinate (m52) at ($(center)+(315:1.7cm)$) {};
\coordinate (m53) at ($(center)+(340:2cm)$) {};
\coordinate (m54) at ($(center)+(315:1.3cm)$) {};
\coordinate (lm5) at ($(center)+(285:1.7cm)$) {};


\coordinate (ln1) at ($(center)+(26:1.1cm)$) {};
\coordinate (ln2) at ($(center)+(112:1.56cm)$) {};
\coordinate (ln3) at ($(center)+(330:1.0cm)$) {};



\begin{tiny}
\tikzstyle{every node}=[inner sep=1pt]
\node at (lm1) {$M_1$};
\node[anchor=east] at (phi_m1) {$\phi|V_{T\setminus N_1}(M_1)$};
\node at (lm2) {$M_2$};
\node[anchor=west] at (phi_m2) {$\phi|V_{T\setminus N_1}(M_2)$};

\node at (lm3) {$M_3$};
\node[anchor=west] at (phi_m3) {$\phi|V_{T\setminus N_1}(M_3)$};

\node at (lm4) {$M_4$};
\node at (lm5) {$M_5$};

\node at (ln1) {$N_1$};
\node at (ln2) {$N_2$};
\node at (ln3) {$N_3$};
\end{tiny}


%m1
\draw[thick] plot [smooth cycle] coordinates {(m11) (m112) (m12) (m13) (m14) (m15)};

%m2
\draw[thick] plot [smooth cycle] coordinates {(m21) (m22) (m23) (m24)};

%m3
\draw[thick] plot [smooth cycle] coordinates {(m31) (m32) (m33) (m34)};


%m4
\draw[thick] plot [smooth cycle] coordinates {(m41) (m42) (m43) (m44)};

%m5
\draw[thick] plot [smooth cycle] coordinates {(m51) (m52) (m53) (m54)};


\draw (0,0) circle (2cm);

\draw[very thick,red,|-|] ([shift=(10:2cm)]0,0) arc (10:30:2cm);
\draw[very thick,red,|-|] ([shift=(35:2cm)]0,0) arc (35:75:2cm);
\draw[very thick,red,|-|] ([shift=(88:2cm)]0,0) arc (88:362:2cm);



\draw[white] (-3.4,-2.5)--(-3.4,-2.3);
\draw[white] (3.8,2.5)--(3.8,2.3);

\end{tikzpicture} 
\caption{\label{fig:T_NM_tree_subwords} 
A conformal model $\phi$ of $G_{ov}$ and contiguous subwords: $\phi|V_{T \setminus M_1}(N_1)$, $\phi|V_{T \setminus M_1}(N_2)$, and $\phi|V_{T \setminus M_1}(N_3)$ (to the left), and $\phi|V_{T \setminus N_1}(M_1)$, $\phi|V_{T \setminus N_1}(M_2)$, and $\phi|V_{T \setminus N_1}(M_3)$ (to the right). We have $\phi_{M_1} \equiv \tau_1N_1\tau_2N_3\tau_3N_2$ and $\phi_{N_1} \equiv M_1M_3M_2$.}
\end{figure}


==> figures/reduct/circle_prime_reduct.tex <==
\begin{figure}[htp!]
\centering
\begin{tikzpicture}[scale=2.1,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]

\coordinate (center) at (0,0) {};
\coordinate (label) at (0,-2.5) {};

\coordinate (s1) at ($(center)+(340:2.0cm)$) {};
\coordinate (s2) at ($(center)+(60:2.0cm)$) {};

\coordinate (s3) at ($(center)+(0:2.0cm)$) {};
\coordinate (s4) at ($(center)+(40:2.0cm)$) {};
\coordinate (s5) at ($(center)+(270:2.0cm)$) {};
\coordinate (s6) at ($(center)+(320:2.0cm)$) {};
\coordinate (s7) at ($(center)+(70:2.0cm)$) {};
\coordinate (s8) at ($(center)+(110:2.0cm)$) {};

\coordinate (s9) at ($(center)+(130:2.0cm)$) {};
\coordinate (s10) at ($(center)+(180:2.0cm)$) {};

\coordinate (s11) at ($(center)+(135:2.0cm)$) {};
\coordinate (s12) at ($(center)+(260:2.0cm)$) {};

\coordinate (s13) at ($(center)+(145:2.0cm)$) {};
\coordinate (s14) at ($(center)+(245:2.0cm)$) {};

\coordinate (s15) at ($(center)+(155:2.0cm)$) {};
\coordinate (s16) at ($(center)+(225:2.0cm)$) {};

\coordinate (s17) at ($(center)+(165:2.0cm)$) {};
\coordinate (s18) at ($(center)+(205:2.0cm)$) {};

\coordinate (s19) at ($(center)+(250:2.0cm)$) {};
\coordinate (s20) at ($(center)+(290:2.0cm)$) {};

\coordinate (s21) at ($(center)+(235:2.0cm)$) {};
\coordinate (s22) at ($(center)+(350:2.0cm)$) {};

\coordinate (s23) at ($(center)+(218:2.0cm)$) {};
\coordinate (s24) at ($(center)+(10:2.0cm)$) {};

\coordinate (s25) at ($(center)+(200:2.0cm)$) {};
\coordinate (s26) at ($(center)+(80:2.0cm)$) {};

\coordinate (p0) at ($(center)+(50:2.0cm)$) {};
\coordinate (p1) at ($(center)+(20:2.0cm)$) {};
\coordinate (p2) at ($(center)+(30:2.0cm)$) {};
\coordinate (p3) at ($(center)+(120:2.0cm)$) {};

\coordinate (t1) at ($(center)+(208:2.0cm)$) {};
\coordinate (t2) at ($(center)+(25:2.0cm)$) {};
\coordinate (t3) at ($(center)+(160:2.0cm)$) {};
\coordinate (t4) at ($(center)+(213:2.0cm)$) {};




\draw (0,0) circle (2cm);

\node[fill=red, circle, inner sep=2.5pt] at (p0) {};
\node[fill=red, circle, inner sep=2.5pt] at (p1) {};
\node[fill=red, circle, inner sep=2.5pt] at (p2) {};
\node[fill=red, circle, inner sep=2.5pt] at (p3) {};

\draw[thick,red,->] (s1) -- (s2);
\draw[thick,red,->] (s3) -- (s4);
\draw[thick,red,->] (s5) -- (s6);
\draw[thick,red,<-] (s7) -- (s8);

\draw[thick,black,->] (s9) -- (s10);
\draw[thick,black,->] (s11) -- (s12);
\draw[thick,black,->] (s13) -- (s14);
\draw[thick,black,->] (s15) -- (s16);
\draw[thick,black,->] (s17) -- (s18);

\draw[thick,black,->] (s19) -- (s20);
\draw[thick,black,->] (s21) -- (s22);
\draw[thick,black,->] (s23) -- (s24);
\draw[thick,black,->] (s25) -- (s26);

\draw[thick,black,->] (t1) -- (t2);
\draw[thick,black,->] (t3) -- (t4);

\end{tikzpicture}

\caption{
\label{fig:circle_prime_reduct}
Construction for an $M$-node $N\in V(\mathcal{T})$. Interesting children of $N$ and the parent of $N$ (when $N\neq R$) are depicted in red.
}
\end{figure}

==> figures/reduct/proper_prime_reduct.tex <==
\begin{figure}[htp!]
\centering
\begin{tikzpicture}[yscale=0.75,xscale=0.5,>=latex,shorten>=-0.2pt,shorten <=-0.2pt]
\coordinate (label) at (1.5,-1) {};

\coordinate (a_v1) at (0,3) {};
\coordinate (a_v2) at (1,3) {};
\coordinate (a_v3) at (2,3) {};
\coordinate (a_v4) at (3,3) {};

\coordinate (b_v1) at (0,0) {};
\coordinate (b_v2) at (1,0) {};
\coordinate (b_v3) at (2,0) {};
\coordinate (b_v4) at (3,0) {};

\coordinate (la_v1) at (0,3.3) {};
\coordinate (la_v2) at (1,3.3) {};
\coordinate (la_v3) at (2,3.3) {};
\coordinate (la_v4) at (3,3.3) {};

\coordinate (lb_v1) at (0,-0.3) {};
\coordinate (lb_v2) at (1,-0.3) {};
\coordinate (lb_v3) at (2,-0.3) {};
\coordinate (lb_v4) at (3,-0.3) {};

\coordinate (tau0) at (3.9,3);
\coordinate (tau1) at (-0.9,0);

\draw[->] (-0.5,3) -- (3.5,3);
\draw[<-] (-0.5,0) -- (3.5,0);

\draw[->,black] (a_v1)--(b_v3);
\draw[->,black] (a_v2)--(b_v1);
\draw[->,black] (a_v3)--(b_v4);
\draw[->,red,very thick] (a_v4)--(b_v2);

\begin{tiny}
\node at (la_v1) {$E^0_1$};
\node at (la_v2) {$E^0_2$};
\node at (la_v3) {$E^0_3$};
\node at (la_v4) {$K^0_{i}$};

\node at (lb_v1) {$E^1_2$};
\node at (lb_v2) {$K^1_{i}$};
\node at (lb_v3) {$E^1_1$};
\node at (lb_v4) {$E^1_3$};
\end{tiny}

\begin{scriptsize}
\node at (label) {(a)};
%\node at (tau0) {$\lambda^0$};
%\node at (tau1) {$\lambda^1$};
\end{scriptsize}
\draw[white] (-1,-1.3)--(0,-1.3);
\end{tikzpicture}
\hspace{0.35cm}
\begin{tikzpicture}[yscale=0.75,xscale=0.5,>=latex,shorten>=-0.2pt,shorten <=-0.2pt]
\coordinate (label) at (0.5,-1) {};
\coordinate (a_v1) at (0,3) {};
\coordinate (a_v2) at (1,3) {};

\coordinate (b_v1) at (0,0) {};
\coordinate (b_v2) at (1,0) {};

\coordinate (la_v1) at (0,3.3) {};
\coordinate (la_v2) at (1,3.3) {};

\coordinate (lb_v1) at (0,-0.3) {};
\coordinate (lb_v2) at (1,-0.3) {};

\coordinate (tau0) at (1.9,3);
\coordinate (tau1) at (-0.9,0);

\draw[->] (-0.5,3) -- (1.5,3);
\draw[<-] (-0.5,0) -- (1.5,0);

\draw[->,black] (a_v1)--(b_v1);
\draw[->,red, very thick] (a_v2)--(b_v2);

\begin{tiny}
\node at (la_v1) {$E^0_1$};
\node at (la_v2) {$K^0_{i}$};

\node at (lb_v1) {$E^1_1$};
\node at (lb_v2) {$K^1_{i}$};
\end{tiny}

\begin{scriptsize}
\node at (label) {(b)};
%\node at (tau0) {$\lambda^0$};
%\node at (tau1) {$\lambda^1$};
\end{scriptsize}
\draw[white] (-1,-1.3)--(0,-1.3);
\end{tikzpicture}
\hspace{0.35cm}
\begin{tikzpicture}[yscale=0.75,xscale=0.5,>=latex,shorten>=-0.2pt,shorten <=-0.2pt]
\coordinate (label) at (0.5,-1) {};
\coordinate (a_v1) at (0,3) {};
\coordinate (a_v2) at (1,3) {};

\coordinate (b_v1) at (0,0) {};
\coordinate (b_v2) at (1,0) {};

\coordinate (la_v1) at (0,3.3) {};
\coordinate (la_v2) at (1,3.3) {};

\coordinate (lb_v1) at (0,-0.3) {};
\coordinate (lb_v2) at (1,-0.3) {};

\coordinate (tau0) at (1.9,3);
\coordinate (tau1) at (-0.9,0);

\draw[->] (-0.5,3) -- (1.5,3);
\draw[<-] (-0.5,0) -- (1.5,0);

\draw[->,black] (a_v1)--(b_v2);
\draw[->,red, very thick] (a_v2)--(b_v1);

\begin{tiny}
\node at (la_v1) {$E^0_1$};
\node at (la_v2) {$K^0_{i}$};

\node at (lb_v1) {$K^1_{i}$};
\node at (lb_v2) {$E^1_1$};
\end{tiny}

\begin{scriptsize}
\node at (label) {(c)};
%\node at (tau0) {$\lambda^0$};
%\node at (tau1) {$\lambda^1$};
\end{scriptsize}
\draw[white] (-1,-1.3)--(0,-1.3);
\end{tikzpicture}
\hspace{0.75cm}
\begin{tikzpicture}[yscale=0.75,xscale=0.5,>=latex,shorten>=-0.2pt,shorten <=-0.2pt]
\coordinate (label) at (6,-1) {};
\coordinate (a_v1) at (0,3) {};
\coordinate (a_v2) at (1,3) {};
\coordinate (a_v3) at (2,3) {};
\coordinate (a_v4) at (3,3) {};
\coordinate (a_v5) at (4,3) {};
\coordinate (a_v6) at (5,3) {};
\coordinate (a_v7) at (6,3) {};
\coordinate (a_v8) at (7,3) {};
\coordinate (a_v9) at (8,3) {};
\coordinate (a_v10) at (9,3) {};
\coordinate (a_v11) at (10,3) {};
\coordinate (a_v12) at (11,3) {};
\coordinate (a_v13) at (12,3) {};


\coordinate (b_v1) at (0,0) {};
\coordinate (b_v2) at (1,0) {};
\coordinate (b_v3) at (2,0) {};
\coordinate (b_v4) at (3,0) {};
\coordinate (b_v5) at (4,0) {};
\coordinate (b_v6) at (5,0) {};
\coordinate (b_v7) at (6,0) {};
\coordinate (b_v8) at (7,0) {};
\coordinate (b_v9) at (8,0) {};
\coordinate (b_v10) at (9,0) {};
\coordinate (b_v11) at (10,0) {};
\coordinate (b_v12) at (11,0) {};
\coordinate (b_v13) at (12,0) {};

\coordinate (la_v1) at (0,3.3) {};
\coordinate (la_v2) at (1,3.3) {};
\coordinate (la_v3) at (2,3.3) {};
\coordinate (la_v4) at (3,3.3) {};
\coordinate (la_v5) at (4,3.3) {};
\coordinate (la_v6) at (5,3.3) {};
\coordinate (la_v7) at (6,3.3) {};
\coordinate (la_v8) at (7,3.3) {};
\coordinate (la_v9) at (8,3.3) {};
\coordinate (la_v10) at (9,3.3) {};
\coordinate (la_v11) at (10,3.3) {};
\coordinate (la_v12) at (11,3.3) {};
\coordinate (la_v13) at (12,3.3) {};

\coordinate (lb_v1) at (0,-0.3) {};
\coordinate (lb_v2) at (1,-0.3) {};
\coordinate (lb_v3) at (2,-0.3) {};
\coordinate (lb_v4) at (3,-0.3) {};
\coordinate (lb_v5) at (4,-0.3) {};
\coordinate (lb_v6) at (5,-0.3) {};
\coordinate (lb_v7) at (6,-0.3) {};
\coordinate (lb_v8) at (7,-0.3) {};
\coordinate (lb_v9) at (8,-0.3) {};
\coordinate (lb_v10) at (9,-0.3) {};
\coordinate (lb_v11) at (10,-0.3) {};
\coordinate (lb_v12) at (11,-0.3) {};
\coordinate (lb_v13) at (12,-0.3) {};

\coordinate (tau0) at (12.9,3);
\coordinate (tau1) at (-0.9,0);


\draw[->,black] (a_v1)--(b_v6);
\draw[->,red,very thick] (a_v2)--(b_v3);
\draw[->,black] (a_v3)--(b_v8);
\draw[->,red,very thick] (a_v4)--(b_v1);
\draw[->,black] (a_v5)--(b_v10);
\draw[->,red,very thick] (a_v6)--(b_v2);
\draw[->,black] (a_v7)--(b_v12);
\draw[->,red,very thick] (a_v8)--(b_v4);
\draw[->,green] (a_v9)--(b_v13);
\draw[->,blue] (a_v10)--(b_v5);
\draw[->,blue] (a_v11)--(b_v7);
\draw[->,blue] (a_v12)--(b_v9);
\draw[->,blue] (a_v13)--(b_v11);

\draw[->] (-0.5,3) -- (12.5,3);
\draw[<-] (-0.5,0) -- (12.5,0);


\tikzstyle{every node}=[inner sep=1pt]
\begin{tiny}
\node at (la_v1) {$L^0_1$};
\node at (la_v2) {$K^0_1$};
\node at (la_v3) {$L^0_2$};
\node at (la_v4) {$K^0_2$};
\node at (la_v5) {$L^0_3$};
\node at (la_v6) {$K^0_3$};
\node at (la_v7) {$L^0_4$};
\node at (la_v8) {$K^0_4$};
\node at (la_v9) {$M^0_{\text{ }}$};
\node at (la_v10) {$M^0_1$};
\node at (la_v11) {$M^0_2$};
\node at (la_v12) {$M^0_3$};
\node at (la_v13) {$M^0_4$};

\node at (lb_v1) {$K^1_2$};
\node at (lb_v2) {$K^1_3$};
\node at (lb_v3) {$K^1_1$};
\node at (lb_v4) {$K^1_4$};
\node at (lb_v5) {$M^1_1$};
\node at (lb_v6) {$L^1_1$};
\node at (lb_v7) {$M^1_2$};
\node at (lb_v8) {$L^1_2$};
\node at (lb_v9) {$M^1_3$};
\node at (lb_v10) {$L^1_3$};
\node at (lb_v11) {$M^1_4$};
\node at (lb_v12) {$L^1_4$};
\node at (lb_v13) {$M^1_{\text{ }}$};
\end{tiny}

\begin{scriptsize}
\node at (tau0) {$\lambda^0$};
\node at (tau1) {$\lambda^1$};
\node at (label) {(d)};
\end{scriptsize}
\draw[white] (-1,-1.3)--(0,-1.3);
\end{tikzpicture}

\caption{
\label{fig:M-node-reduct}
Figures (a),(b), and (c) show the extended reducts of $N_i$ for the case when $N_i$ is prime, paralell, and serial, respectively.  
Figure (d) shows the reduct of $N$ for the case when $N$ is prime: $N$ has 4 important children $N_1,\ldots,N_4$ with the reducts $K_1,\ldots,K_4$.} 
\end{figure}


==> figures/reduct/single_metachord.tex <==
\begin{figure}[htp!]
\centering
\begin{tikzpicture}[scale=1,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]

\coordinate (center) at (0,0) {};
\coordinate (label) at (0,-2.5) {};

\coordinate (s1) at ($(center)+(300:2.0cm)$) {};
\coordinate (s2) at ($(center)+(60:2.0cm)$) {};
\coordinate (s3) at ($(center)+(0:2.0cm)$) {};
\coordinate (s4) at ($(center)+(140:2.0cm)$) {};
\coordinate (s5) at ($(center)+(100:2.0cm)$) {};
\coordinate (s6) at ($(center)+(220:2.0cm)$) {};
\coordinate (s7) at ($(center)+(180:2.0cm)$) {};
\coordinate (s8) at ($(center)+(270:2.0cm)$) {};


\draw (0,0) circle (2cm);

\draw[thick,red,->] (s1) -- (s2);
\draw[thick,black,->] (s3) -- (s4);
\draw[thick,black,->] (s5) -- (s6);
\draw[thick,black,->] (s7) -- (s8);


\end{tikzpicture}
\caption{
\label{fig:single_metachord}
Construction in the case there is a single $CA$-module $S$ (red) satisfying $S\cap U \neq \emptyset$. }
\end{figure}

==> figures/structure_descr/admissible_models_correspondence.tex <==
\begin{figure}[ht]
\begin{tikzpicture}[scale=0.8,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\tikzstyle{every node}=[rectangle,minimum size=15pt,inner sep=0.5,draw];
  \begin{scriptsize}
  \node (M) at (4.0,7.5) {$S_i$};
  \node (v1) at (0.5,6) {$A_1 = \{v_1\}$};
  \node (A) at (3,6) {$A_2$};
  \node (B) at (5.5,6) {$A_3$};
  \node (v9) at (8,6) {$A_4 = \{v_9\}$};
  \node (v2) at (0.5,4.5) {$B_1 = \{v_2\}$};
  \node (C) at (2.5,4.5) {$B_2$};
  \node (D) at (4,4.5) {$B_3$};
  \node (v7) at (5.5,4.5) {$\{v_7\}$};
  \node (v8) at (7,4.5) {$\{v_8\}$};
  \node (v3) at (1.8,3) {$\{v_3\}$};
  \node (v4) at (2.8,3) {$\{v_4\}$};
  \node (v5) at (4.0,3) {$\{v_5\}$};
  \node (v6) at (5,3) {$\{v_6\}$};
 
\end{scriptsize}
\tikzstyle{every node}=[square,minimum size=15pt,inner sep=0.5,draw];
\path (M) edge (v1); 
\path (M) edge (A); 
\path (M) edge (B); 
\path (M) edge (v9); 
\path (A) edge (v2); 
\path (A) edge (C); 
\path (A) edge (D); 
\path (B) edge (v7); 
\path (B) edge (v8); 
\path (C) edge (v3); 
\path (C) edge (v4); 
\path (D) edge (v5); 
\path (D) edge (v6); 

\draw[-,white] (-0.5,1) -- (0,1);
\end{tikzpicture}
\hspace{0.5cm}
\begin{tikzpicture}[scale=0.75,>=latex,shorten>=-0.2pt,shorten <=-0.2pt]
\coordinate (a_v1) at (0,3) {};
\coordinate (a_v2) at (1,3) {};
\coordinate (a_v3) at (2,3) {};
\coordinate (a_v4) at (2.5,3) {};
\coordinate (a_v5) at (3.4,3) {};
\coordinate (a_v6) at (3.8,3) {};
\coordinate (a_v7) at (5.2,3) {};
\coordinate (a_v8) at (5.8,3) {};
\coordinate (a_v9) at (7,3) {};

\coordinate (b_v2) at (7,0) {};
\coordinate (b_v4) at (6,0) {};
\coordinate (b_v3) at (5.5,0) {};
\coordinate (b_v6) at (4.5,0) {};
\coordinate (b_v5) at (4.1,0) {};
\coordinate (b_v9) at (2.5,0) {};
\coordinate (b_v1) at (1.5,0) {};
\coordinate (b_v8) at (0.6,0) {};
\coordinate (b_v7) at (0,0) {};

\coordinate (lb_v2) at (7,-0.3) {};
\coordinate (lb_v4) at (6,-0.3) {};
\coordinate (lb_v3) at (5.5,-0.3) {};
\coordinate (lb_v6) at (4.5,-0.3) {};
\coordinate (lb_v5) at (4.1,-0.3) {};
\coordinate (lb_v9) at (2.5,-0.3) {};
\coordinate (lb_v1) at (1.5,-0.3) {};
\coordinate (lb_v8) at (0.6,-0.3) {};
\coordinate (lb_v7) at (0,-0.3) {};


\coordinate (tau0) at (7.9,3);
\coordinate (tau1) at (-0.9,0);


\tikzstyle{every node}=[inner sep=2pt,fill=white]

\draw[fill=gray!30, draw=none] (-0.2,3) -- (0.2,3) -- (1.7,0) -- (1.3,0) -- cycle;
\coordinate (m_A1) at (0,3.3) {};

\draw[fill=gray!30, draw=none] (0.7,3) -- (4.1,3) -- (7.3,0) -- (3.8,0) -- cycle;
\coordinate (m_A) at (5.55,-0.3) {};

\draw[fill=gray!30, draw=none] (4.9,3) -- (6.1,3) -- (0.9,0) -- (-0.3,0) -- cycle;
\coordinate (m_A3) at (5.5,3.3) {};

\draw[fill=gray!30, draw=none] (6.7,3) -- (7.3,3) -- (2.8,0) -- (2.2,0) -- cycle;
\coordinate (m_A4) at (7,3.3) {};

\draw[fill=gray!80, draw=none] (0.7,3) -- (1.3,3) -- (7.3,0) -- (6.7,0) -- cycle;
\coordinate (m_B1) at (1,3.3) {};
\draw[fill=gray!80, draw=none] (1.8,3) -- (2.7,3) -- (6.2,0) -- (5.3,0) -- cycle;
\coordinate (m_B2) at (2.25,3.3) {};
\draw[fill=gray!80, draw=none] (3.2,3) -- (4,3) -- (4.7,0) -- (3.9,0) -- cycle;
\coordinate (m_B3) at (3.7,3.3) {};

\draw[<-] (a_v1)--(b_v1);
\draw[->] (a_v2)--(b_v2);
\draw[<-] (a_v3)--(b_v3);
\draw[->] (a_v4)--(b_v4);
\draw[<-] (a_v5)--(b_v5);
\draw[->] (a_v6)--(b_v6);
\draw[<-] (a_v7)--(b_v7);
\draw[->] (a_v8)--(b_v8);
\draw[->] (a_v9)--(b_v9);

\draw[->] (-0.5,3) -- (7.5,3);
\draw[<-] (-0.5,0) -- (7.5,0);


\tikzstyle{every node}=[inner sep=1pt]
\begin{footnotesize}
\node at (lb_v1) {$v_1$};
\node at (lb_v2) {$v_2$};
\node at (lb_v3) {$v_3$};
\node at (lb_v4) {$v_4$};
\node at (lb_v5) {$v_5$};
\node at (lb_v6) {$v_6$};
\node at (lb_v7) {$v_7$};
\node at (lb_v8) {$v_8$};
\node at (lb_v9) {$v_9$};
\node at (tau0) {$\mu^0$};
\node at (tau1) {$\mu^1$};
\node at (m_A1) {$A_1$};
\node at (m_B1) {$B_1$};
\node at (m_B2) {$B_2$};
\node at (m_B3) {$B_3$};
\node at (m_A3) {$A_3$};
\node at (m_A4) {$A_4$};
%\node at (m_v9) {$\{v_9\}$};

\end{footnotesize}

%gorna kopia
\coordinate (a_v1) at (0,5) {};
\coordinate (a_v2) at (1,5) {};
\coordinate (a_v3) at (2,5) {};
\coordinate (a_v4) at (2.5,5) {};
\coordinate (a_v5) at (3.4,5) {};
\coordinate (a_v6) at (3.8,5) {};
\coordinate (a_v7) at (5.2,5) {};
\coordinate (a_v8) at (5.8,5) {};
\coordinate (a_v9) at (7,5) {};


\coordinate (b_v2) at (7,8) {};
\coordinate (b_v4) at (6,8) {};
\coordinate (b_v3) at (5.5,8) {};
\coordinate (b_v6) at (4.5,8) {};
\coordinate (b_v5) at (4.1,8) {};
\coordinate (b_v9) at (2.5,8) {};
\coordinate (b_v1) at (1.5,8) {};
\coordinate (b_v8) at (0.6,8) {};
\coordinate (b_v7) at (0,8) {};

\coordinate (la_v1) at (0,4.7) {};
\coordinate (la_v2) at (1,4.7) {};
\coordinate (la_v3) at (2,4.7) {};
\coordinate (la_v4) at (2.5,4.7) {};
\coordinate (la_v5) at (3.4,4.7) {};
\coordinate (la_v6) at (3.8,4.7) {};
\coordinate (la_v7) at (5.2,4.7) {};
\coordinate (la_v8) at (5.8,4.7) {};
\coordinate (la_v9) at (7,4.7) {};

\coordinate (mu0) at (-0.9,5);
\coordinate (mu1) at (7.9,8);

\tikzstyle{every node}=[inner sep=2pt,fill=white]

\draw[fill=gray!30, draw=none] (-0.2,5) -- (0.2,5) -- (1.7,8) -- (1.3,8) -- cycle;
\coordinate (m_A1) at (1.5,8.3) {};

\draw[fill=gray!30, draw=none] (0.7,5) -- (4.1,5) -- (7.3,8) -- (3.8,8) -- cycle;
%\coordinate (m_A) at (2.4,4.7) {};

\draw[fill=gray!30, draw=none] (4.9,5) -- (6.1,5) -- (0.9,8) -- (-0.3,8) -- cycle;
\coordinate (m_A2) at (0.3,8.3) {};

\draw[fill=gray!30, draw=none] (6.7,5) -- (7.3,5) -- (2.8,8) -- (2.2,8) -- cycle;
\coordinate (m_A3) at (2.5,8.3) {};

\draw[fill=gray!80, draw=none] (0.7,5) -- (1.3,5) -- (7.3,8) -- (6.7,8) -- cycle;
\coordinate (m_B1) at (7,8.3) {};
\draw[fill=gray!80, draw=none] (1.8,5) -- (2.7,5) -- (6.2,8) -- (5.3,8) -- cycle;
\coordinate (m_B2) at (5.75,8.3) {};
\draw[fill=gray!80, draw=none] (3.2,5) -- (4,5) -- (4.7,8) -- (3.9,8) -- cycle;
\coordinate (m_B3) at (4.3,8.3) {};


\draw[->] (a_v1)--(b_v1);
\draw[<-] (a_v2)--(b_v2);
\draw[->] (a_v3)--(b_v3);
\draw[<-] (a_v4)--(b_v4);
\draw[->] (a_v5)--(b_v5);
\draw[<-] (a_v6)--(b_v6);
\draw[->] (a_v7)--(b_v7);
\draw[<-] (a_v8)--(b_v8);
\draw[<-] (a_v9)--(b_v9);

\draw[<-] (-0.5,5) -- (7.5,5);
\draw[->] (-0.5,8) -- (7.5,8);

\tikzstyle{every node}=[inner sep=1pt]
\begin{footnotesize}
\node at (la_v1) {$v_1$};
\node at (la_v2) {$v_2$};
\node at (la_v3) {$v_3$};
\node at (la_v4) {$v_4$};
\node at (la_v5) {$v_5$};
\node at (la_v6) {$v_6$};
\node at (la_v7) {$v_7$};
\node at (la_v8) {$v_8$};
\node at (la_v9) {$v_9$};
\node at (mu0) {$\tau^1$};
\node at (mu1) {$\tau^0$};
\node at (m_A1) {$A_1$};
\node at (m_A2) {$A_3$};
\node at (m_A3) {$A_4$};
\node at (m_B1) {$B_1$};
\node at (m_B2) {$B_2$};
\node at (m_B3) {$B_3$};
\end{footnotesize}

\end{tikzpicture}
\caption{\label{fig:admissible_models_modular_decomposition} The modular decomposition $\mathcal{M}(S_i,{\sim})$ of $(S_i,{\sim})$ (to the left) 
and two admissible models for $\mathbb{S}_i$ (to the right).
Module $S_i$ is prime and hence $(S_i,{\sim_{S_i}})$ has two transitive orientations.
Module $A_2$ is serial with three children and hence $(A_2,{\sim_{A_2}})$ has $3!$ transitive orientations.
The remaining non-trivial modules $A_3, B_2, B_3$ are parallel and each of them has one empty transitive orientation.
Hence, the metaedge $\mathbb{S}_i$ has $12$ different admissible models, corresponding to $12=2 \cdot 3!$ transitive orientations of $(S_i,{\sim})$.
The admissible models $(\tau^0,\tau^1)$ and $(\mu^0,\mu^1)$ for $\mathbb{S}_i$ 
correspond to the transitive orientations $\prec_{\tau}$ and $\prec_{\mu}$ of $(S_i,{\sim})$.
The orientation $(S_i,\prec_{\tau}$) is obtained from the orientation 
$A_3 \prec_{\tau} A_1,\ A_3 \prec_{\tau} A_2,\ A_4 \prec_{\tau} A_2$ of $(S,{\sim_{S_i}})$ 
and the orientation $B_3 \prec_{\tau} B_2 \prec_{\tau} B_1$ of $(A_2,{\sim_{A_2}})$. 
The orientation $(S_i,\prec_{\mu}$) is obtained 
from the orientation $A_1 \prec_{\mu} A_3,\ A_2 \prec_{\mu} A_3,\ A_2 \prec_{\mu} A_4$ of $(S,{\sim_{S_i}})$ 
and the orientation $B_1 \prec_{\mu} B_2 \prec_{\mu} B_3$ of $(A_2,{\sim_{A_2}})$.
}
\end{figure}

